Optimizing Multispectral Object Detection: A Bag of Tricks and Comprehensive Benchmarks

Multispectral object detection, utilizing RGB and TIR (thermal infrared) modalities, is widely recognized as a challenging task. It requires not only the effective extraction of features from both modalities and robust fusion strategies, but also the ability to address issues such as spectral discrepancies, spatial misalignment, and environmental dependencies between RGB and TIR images. These challenges significantly hinder the generalization of multispectral detection systems across diverse scenarios. Although numerous studies have attempted to overcome these limitations, it remains difficult to clearly distinguish the performance gains of multispectral detection systems from the impact of these "optimization techniques". Worse still, despite the rapid emergence of high-performing single-modality detection models, there is still a lack of specialized training techniques that can effectively adapt these models for multispectral detection tasks. The absence of a standardized benchmark with fair and consistent experimental setups also poses a significant barrier to evaluating the effectiveness of new approaches. To this end, we propose the first fair and reproducible benchmark specifically designed to evaluate the training "techniques", which systematically classifies existing multispectral object detection methods, investigates their sensitivity to hyper-parameters, and standardizes the core configurations. A comprehensive evaluation is conducted across multiple representative multispectral object detection datasets, utilizing various backbone networks and detection frameworks. Additionally, we introduce an efficient and easily deployable multispectral object detection framework that can seamlessly optimize high-performing single-modality models into dual-modality models, integrating our advanced training techniques.

==> Final/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Final/sections/comments.tex <==
%%%INTRO

% A large number of real world applications consume unstructured (non-Euclidean) data. To overcome the shortcomings of CNNs, Graph Convolutional Networks (GCNs) provide solutions for unstructured data processing. These solutions have found an increasing interest in a variety of applications
% Deep learning is hailed today for achieving state-of-the-art results in a wide range of fields. While their success is unparalleled with Euclidean/structured data, deep learning   
% Problem in CNNs also occur in GCNs.
% Vanishing gradient problem and over-smoothing in Graph Neural Network limits the scalability. Laplacian smoothing. Memory inefficent. receptive field.
% Resolve those problem by the ideas from CNNs 


%%%RELATED WORK

% \begin{comment}
% 1) Importance of graphs and GCNs
% 2) Applications of graphs (leading to 3d point clouds)
% 3) Limitations of GCNs (e.g. depth: oversmoothing, etc.)
% 3) Inspired by 2D, dilation, residual, dense
% spectral method and spatial method.\\
% spatial-based graph convolution network.\\
% GNN general applications and applications in computer vision\\
% Node-level (segmentation), Edge-level, Graph-level (classification)\\
% Related works that attempts to make GNNs deeper. GCN \cite{kipf2016semi} - 2 layers, GraphSAGE - 2 layers \cite{hamilton2017inductive}, Highway GCN \cite{rahimi2018semi} - 4 layers,  Jump Knowledge Network \cite{xu2018representation} - 6 layers, GLN \cite{pham2017column} - 10 layers, \\
% we study our methods on point cloud datasets, point cloud related works...
% \\
% \vspace{3pt}\noindent\textbf{Contributions.~}
% \end{comment}


%%%METHODOLOGY

% \begin{comment}
% In this section, We first define representation learning on graphs using graph neural networks (GNNs); especially, graph convolutional networks (GCNs) \bibi{You do not have to redefine this multiple times. Define it once in the abstract and use GCNs all over.} (See \ref{sec:defineGCN}). And then we show how to bring concepts, including residual learning \ref{sec:ResGCN}, dense connections \ref{sec:DenseGCN} and dilated convolutions \ref{sec:dilation}, from convolutional neurak networks (CNNs) to GCNs. At the end, we introduce how to use proposed GCNs frameworks to process point clouds \ref{sec:PCGCN} which are fundamentally irregular and non-grid data.
% \subsection{Representation Learning on Graphs} \label{sec:defineGCN}
% \vspace{3pt}\noindent\textbf{Definition of graph.~} A Graph $\mathcal{G}$ is represented by a tuple $\mathcal{G}=(\mathcal{V}, \mathcal{E})$ where $\mathcal{V}$ is the set of vertices and $\mathcal{E}$ is the set of edges representing the connectivity between vertices $v \in \mathcal{V}$. For $e_{i,j} \in \mathcal{E}$, vertices $v_i$ and $v_j$ are connected to each other with an edge $e_{i,j}$.
% \end{comment}

% \begin{equation} \label{eq1}
% \begin{split}
% \mathcal{G}_{l+1}=\mathcal{F}(\mathcal{G}_{l}, \mathcal{W}_l).
% \end{split}
% \end{equation}

%%%EXPERIMENTS

% \begin{table}[]
% \centering
% \begin{tabular}{c|cc|cc}
% \toprule
% & \multicolumn{2}{c}{\textbf{Vanilla}} & \multicolumn{2}{c}{\textbf{Reference (ours)}} \\
%  & \textbf{IoU} & \textbf{accuracy} & \textbf{IoU} & \textbf{accuracy} \\ \midrule
% Area 1           &      &    & 70.28     & 0.892      \\
% Area 2           &      &    & 43.40     & 0.791      \\
% Area 3           &      &    & 67.20     & 0.892      \\
% Area 4           &      &    & 51.39     & 0.845      \\
% Area 5           &      &    & 52.18     & 0.854     \\
% Area 6           &      &    & 74.84     & 0.907      \\ \midrule
% \textbf{mIoU}    &      &    & \textbf{59.88} & \textbf{0.863}   \\
% \bottomrule
% \end{tabular}
% \vspace{6pt}
% \caption{Results across all areas with our reference network with 28 layers, residual connections and dilated convolutions.}
% \label{tbl:ours_all_areas}
% \end{table}


%                                   &        & 48.93 & -3.56 & \checkmark  & \res &            &            &  4 & 64 & 28 \\


%%%CONCLUSION

% dilation can help and it does not increase number of parameters
% different aggregation function and updated function \\
% adapt other operators, e.g. deformable convolution \cite{} \\
% different distance measures to construct $k$-nn graph\\
% better dilated rate schedule and the size of hidden unit of GCNs\\
% dataset augmentation
% differet k for different layers
